Efficient Conformance Checking using Approximate Alignment Computation with Tandem Repeats

Conformance checking encompasses a body of process mining techniques which aim to find and describe the differences between a process model capturing the expected process behavior and a corresponding event log recording the observed behavior. Alignments are an established technique to compute the distance between a trace in the event log and the closest execution trace of a corresponding process model. Given a cost function, an alignment is optimal when it contains the least number of mismatches between a log trace and a model trace. Determining optimal alignments, however, is computationally expensive, especially in light of the growing size and complexity of event logs from practice, which can easily exceed one million events with traces of several hundred activities. A common limitation of existing alignment techniques is the inability to exploit repetitions in the log. By exploiting a specific form of sequential pattern in traces, namely tandem repeats, we propose a novel approximate technique that uses pre- and post-processing steps to compress the length of a trace and recomputes the alignment cost while guaranteeing that the cost result never under-approximates the optimal cost. In an extensive empirical evaluation with 50 real-life model log pairs and against six state-of-the-art alignment techniques, we show that the proposed compression approach systematically outperforms the baselines by up to an order of magnitude in the presence of traces with repetitions, and that the cost over-approximation, when it occurs, is negligible.

==> tex/ProofParallel.tex <==
\begin{algorithm}[!h]
{
    \SetKwInOut{Input}{input}
    \Input{Reduced event log $\redLog$; Reductions $\reductions$;  Reduced DAFSA $\redDafsa$; Reachability Graph $\rg$}
    $\extendedAlignments \leftarrow \{\}$\;
    \For{$t\in\logL$}
    {
        $\trReductions = (\redTrace,\additionalCostF,\redReps,\trPositions) \leftarrow \reductions(t)$\;
        $\alignment\leftarrow\alignments(\trReductions)$\;
        $\position\leftarrow 1$\;
        $\extendedAlignment \leftarrow \langle\rangle$\;
        \While{$\position<\left|\alignment\right|$}
        {
            \uIf{$\position\in\dom(\trPositions)$}
            {
                $\Pairs \leftarrow \langle\rangle$\;                                
                %OLD:                
                %$\firstCopy \leftarrow \langle\sync=\alignment(\secondPos) \mid \secondPos\in\seq(1,\left|\alignment\right|) \tpos(\alignment,\secondPos)\in \seq(\position,\position+\trPositions(\position)-1) \land \text{sort in asc. order with } \secondPos\rangle$\;
                %$\secondCopy \leftarrow \langle\sync=\alignment(\secondPos) \mid \secondPos\in\seq(1,\left|\alignment\right|) \tpos(\alignment,\secondPos)\in \seq(\position+\trPositions(\position)-1,\position+2*\trPositions(\position)-1) \land \text{sort in asc. order with } \secondPos\rangle$
                $\firstCopyEnd \leftarrow \maxF(\secondPos\in\seq(\position,\left|\alignment\right|)\mid\tpos(\alignment,\secondPos)=\position+\trPositions(\position)-1)$\;
                $\secondCopyEnd \leftarrow \maxF(\secondPos\in\seq(\firstCopyEnd+1,\left|\alignment\right|)\mid\tpos(\alignment,\secondPos)=\firstCopyEnd+\trPositions(\position)-1)$\;
                $\posSecExtend\leftarrow \firstCopyEnd+1$\;
                %\lWhile{$\op(\alignment(\posSecExtend))=\rhide$}{$\posSecExtend \leftarrow \posSecExtend + 1$                  }                
                \For{$\posFirstExtend \in \seq(\position,\firstCopyEnd)$}
                {                    
                    \lIf{$\op(\alignment(\posFirstExtend))=\rhide$}{Continue}                    
                    \If{$\op(\alignment(\posFirstExtend))=\op(\alignment(\posSecExtend))=\match$\label{ln:condIsRepeatable}}
                    {
                        $\Pairs \leftarrow \Pairs \tieconcat (\posFirstExtend,\posSecExtend)$\;                    
                    }
                    \lDo{$\op(\secondCopy(\posSecExtend))=\rhide$}{$\posSecExtend \leftarrow \posSecExtend + 1$                }
                }
                %OLD:                
                %\uIf{$\Pairs=\langle\rangle$\label{ln:NoMatchFound}}
                %{
                %    $\copyExtend \leftarrow \langle (\lhide,a_{\dafsa},\perp) \mid  \secondPos\in\seq(1,\left|\firstCopy\right|) \land a_{\dafsa}=\fnSyncDFA(\firstCopy(\secondPos)) \land \op(\firstCopy(\secondPos))\neq\rhide \land \text{sort in  asc. order with }\secondPos \rangle$\;
                %}
                %\Else
                %{
                %OLD:$\copyExtend \leftarrow \pref(\secondCopy,\posSecExtend) \oplus \suff(\firstCopy,\posExtend)$\;
                $\copyExtend \leftarrow \{\secondPos \rightarrow \langle\rangle \mid \secondPos \in \seq(1,\trPositions(\position))\}$\;                    
                \For{$(\startPos,\ePos)\in\Pairs$\label{ln:iteratePairs}}
                {
                    %$\cycle \leftarrow \suff(\firstCopy,\position_1) \tieconcat \pref(\secondCopy,\position_2)$\;
                    $\firstMarking \leftarrow \outTr{\T(\fnSyncRG(\alignment(\startPos)))}$\;
                    %$\secondMarking \leftarrow \inTr{\T(\fnSyncRG(\alignment(\ePos)))}$\;
                    \For{$\secondPos\in\seq(\startPos,\ePos)$}
                    {
                        %$\sync\leftarrow\alignment(\secondPos)$\;                            
                        %\lIf{$\op(\alignment(\secondPos))=\lhide\lor\nexists p\in\firstMarking : p\in\inTr{\T(\fnSyncRG(\alignment(\secondPos)))}$}{Continue}
                        \lIf{$\nexists p\in\firstMarking : p\in\inTr{\T(\fnSyncRG(\alignment(\secondPos)))}$}{Continue}
                        $\firstMarking \leftarrow \outTr{\T(\fnSyncRG(\sync))}$\;
                        \lIf{$\op(\alignment(\secondPos))=\match\land\exists (s,e)\in\Pairs:s=\secondPos\lor e=\secondPos$}{Remove $(s,e)$ from $\Pairs$}
                        \lIf{$\secondPos\leq\firstCopyEnd$}{$\posTR\leftarrow \tpos(\alignment,\secondPos)-\tpos(\alignment,\position)$}
                        \lElse{$\posTR\leftarrow\tpos(\alignment,\secondPos)-\tpos(\alignment,\firstCopyEnd)$}
                        $\copyExtend(\posTR)\leftarrow\copyExtend(\posTR)\tieconcat\sync$\;                                                        
                    }     
                }
                \lFor{$\secondPos \in \seq(1,\trPositions(\position)) \mid \copyExtend(\secondPos)=\langle\rangle$}
                    {$\copyExtend(\secondPos)\leftarrow\copyExtend(\secondPos)\tieconcat(\lhide,\fnSyncDFA(\filterSyncDFA(\alignment)(\secondPos+\position)),\perp)$}        
                %}
                %OLD:                
                %$\extendedAlignment \leftarrow \extendedAlignment \tieconcat \firstCopy$\;
                %\lFor{$\reps \in \seq(1,\additionalCostF(\position))$}{$\extendedAlignment \leftarrow \extendedAlignment \tieconcat \copyExtend$}
                %$\extendedAlignment\leftarrow\extendedAlignment\tieconcat\secondCopy$\;
                %$\position\leftarrow\position+\left|\firstCopy\tieconcat\secondCopy\right|$\;
                \lFor{$\secondPos\in\seq(\position,\firstCopyEnd)$}{$\extendedAlignment\leftarrow\extendedAlignment\tieconcat\alignment(\secondPos)$}
                \For{$\reps \in \seq(1,\additionalCostF(\position))$}
                {\lFor{$\secondPos\in\seq(1,\trPositions(\position))$}{$\extendedAlignment \leftarrow \extendedAlignment \tieconcat \copyExtend(\secondPos)$}}
                \lFor{$\secondPos\in\seq(\firstCopyEnd+1,\secondCopyEnd)$}{$\extendedAlignment \leftarrow \extendedAlignment\tieconcat \alignment(\secondPos)$}
                $\position \leftarrow \secondCopyEnd+1$\;
            }
            \Else
            {
                $\extendedAlignment \leftarrow \extendedAlignment \tieconcat \alignment(\position)$\;
                $\position\leftarrow\position+1$\;            
            }        
        }
        $\extendedAlignments \leftarrow \extendedAlignments \cup \{t\rightarrow\extendedAlignment\}$\;    
    }
    \Return{$\extendedAlignments$}\;
    \caption{Extending reduced Alignments}\label{alg:ExtendRedAlignments}       
}
\end{algorithm}

Proof of Over approximation

\begin{lemma}[An extended alignment is a proper alignment]\label{lemma:properAlignment}
Given a trace $t\in\logL$, the alignment $\extendedAlignment$, returned by Alg.~\ref{alg:ExtendRedAlignments}, is a proper alignment. 
Thus, the following two properties hold for $\extendedAlignment$:
\begin{compactenum}
  \item\label{prop:two} the arcs in the synchronizations related to the reachability graph forms a path through the reachability graph, i.e., for $\path=\fnSyncRG(\filterSyncRG(\extendedAlignment))$ holds $\src(\path(1)=\rgSource \land \tgt(\path(\left|\path\right|))\in\rgFinStates \land \forall \position\in\seq(1,\left|\path\right|-1) : \tgt(\path(\position))=\src(\path(\position+1))$, and 
    \item\label{prop:one} the labels in the synchronizations related to the DAFSA represent the trace, i.e. $\lbl(\filterSyncDFA(\extendedAlignment))=t$.
\end{compactenum}
\end{lemma}

\begin{proof}
We probe the two properties below:

	\begin{enumerate} 
		\item a
		
		
		\item a
	\end{enumerate} 
\end{proof}



For the proof of lemma~\ref{lemma:properAlignment}, we will particularly relate the extended alignment $\extendedAlignment$ with the reduced alignment $\alignment$ linked with trace $t$, i.e. $\alignment = \alignments(\reductions(t)=(\redTrace,\additionalCostF,\redReps,\trPositions))$. 
The reduced alignment $\alignment$ both properly represents the trace labels of the reduced trace $\redTrace$ as well as forms a path through the reachability graph, because it is checked in the condition in line~\ref{ln:condOptimality} of Alg.~\ref{alg:BinarySearchAlignments}. 
%For proving 
The difference between $t$ and $\redTrace$ is recorded in the function $\trPositions$ in Alg.~\ref{alg:reduceLog} as every tandem repeat starting at position $i\in\dom(\trPositions)$ with length $\trPositions(i)$ is reduced to only two copies present in $\redTrace$. The additional cost function $\additionalCostF$ links each tandem repeat to the amount of reduced repetitions, i.e. $k=\additionalCostF(i)$. In Alg.~\ref{alg:ExtendRedAlignments}, we insert a sequence of synchronizations $\copyExtend$ after the first aligned copy of each tandem repeat $\firstCopy$ for $k$-amount of times and before the second copy $\secondCopy$ of the aligned tandem repeat. 
Thus for proving the two properties of lemma~\ref{lemma:properAlignment}, we only need to investigate, if sequence $\copyExtend$ adds the same trace labels as $\firstCopy$ and if the added arcs form a valid path from $\firstCopy$ to $\secondCopy$.
We detect the cases, where a label of the tandem repeat can be repeated in both copies in line~\ref{ln:condIsRepeatable} while moving synchronously through $\firstCopy$ and $\secondCopy$. We record the positions of the repeated label in $\posFirstExtend$ and $\posSecExtend$, respectively, and add them to a list $\pairs$ of repeatable label positions.
In the case that no label of the tandem repeat can be matched in both copies (i.e. when $\Pairs$ is empty in Line~\ref{ln:NoMatchFound}), $\copyExtend$ consists of all $\lhide$-synchronizations for each trace label in the sequence of the first tandem repeat, i.e. $\seq(\position,\firstCopyEnd)$. That way, inserting $\copyExtend$ does not change the path of $\alignment$ through the reachability graph and all missing trace labels are inserted.
In the case that one or more repeating labels can be found, each pair of repeating labels will relate to two $\match$-synchronizations, one in the first and one in the second copy of the aligned tandem repeat.
Since in this work we only consider uniquely-labelled workflow nets, it follows that both matches relate to the same transition and thus the arcs of the reachability graph in between the two matches form a loop. 
%OLD:
%In that case, we construct $\copyExtend$ as the prefix of $\secondCopy$ including the matching label to finish the loop after $\firstCopy$ and then add the suffix of $\firstCopy$ to restart the loop, which concludes in $\secondCopy$. Adding a copy of $\copyExtend$ any number of copies in between $\firstCopy$ and $\secondCopy$ thus results in another viable path over the reachability graph since we just add another traversal of the discovered looping arcs.
However, not all arcs in between the two matches will be a part of that loop since process models can also have transitions that can be executed in parallel and thus will not effect the loop. We identify the repeating subsequence in between the two matches by following the sub-marking $\firstMarking$ after the transition of the Petri net related to the arc of the reachability graph of the first match. We then traverse every synchronization for each pair $(\startPos,\ePos)$ from $\alignment(\startPos)$ up to and including $\alignment(\ePos)$. We add each synchronization to the loop, where the corresponding transition in the Petri net that has at least one place of $\firstMarking$ in its pre-set and then change $\firstMarking$ to the post-set of the transition.
This method will identify a repeatable path through the process model from the transition of $\alignment(\startPos)$ to the transition of $\alignment(\ePos)$ and the sub-marking after $\alignment(\startPos)$ will be equal to the sub-marking after $\alignment(\ePos)$. This path is a valid path through the process model, since the net is free choice, i.e. if the loop is inside a parallel block, then the loop will be contained inside the parallel block fully,  

This case also adds all missing tandem repeat labels, since both $\firstCopy$ and $\secondCopy$ align the same trace labels of the tandem repeat and $\copyExtend$ contains all trace labels of $\secondCopy$ up to and including $\posSecExtend$ and then all trace labels from $\firstCopy$ after $\posExtend$. Since $\posExtend$ and $\posSecExtend$ point to the same trace label, it follows that $\copyExtend$ covers all trace labels of the tandem repeat.
It follows that $\extendedAlignment$ fulfils both properties of lemma~\ref{lemma:properAlignment} and is a proper alignment for trace $t$, which always over-approximates the optimal cost.

As a result of the Lemma~\ref{lemma:properAlignment}, every extended alignment will never under estimate the minimal cost of an alignment. 

\begin{proposition} The cost of an extended alignment is minimal or higher
\end{proposition}

==> tex/TauRemovalCorrection.tex <==
textcolor{red}{}
\section{Correction of the tau-removal algorithm}

\subsection{Expanding a Petri net to its $\tau$-less reachability graph}


\begin{algorithm}[tbp]{
  \SetKwInOut{Input}{input}
  \SetKwProg{Fn}{Function}{}{}
  \vspace{0.5em}
  \begin{compactitem}
   \item[$\triangleright$] insert the following block after line 31
  \end{compactitem}
  \vspace{-0.8em}
  \begin{mdframed}[userdefinedwidth=0.9\textwidth,backgroundcolor=lightgray!20] 
   \begin{algorithmic}[0]
    \begin{compactitem}
     \Indentp{-2em}
     \item[$\triangleright$] Handle a $\tau$-arc from the initial to the final marking
    \end{compactitem}
    \Indentp{-1em}
    \If{$m_1=\initMarking$}
    {
        $\finalMarkings\leftarrow\finalMarking\cup\initMarking$\;
        }  	
   \end{algorithmic}
  \end{mdframed}
 \caption{Remove Tau Transitions - Revision 1}\label{alg:remTauRev1}
 }
\end{algorithm}

\begin{algorithm}[h]{
  \SetKwProg{Fn}{Function}{}{}
 \Fn{$\replaceTauBack((m_1,\tau,m_f) \in \arcs_{\reachGraph})$ \tcp{Function for replacing a given $\tau$ arc backwards}}
 {
    \tcp{If there is a tau-labeled arc from the initial to the final marking, add the initial marking to the set of final markings.}    
    \uIf{$m_1=\initMarking$}{$\finalMarkings\leftarrow\finalMarking\cup\initMarking$}     
     %\tcp{For each incoming arc of the source marking of the input $\tau$ arc}
     \tcp{Replace incoming arcs of $m_1$ with arcs from the predecessors of $m_1$ to $m_f$}
     \For{$(m_2,l,m_1) \in \inT{m_1} \mid l \neq \tau$}
     {
        $\arcs_{\reachGraph} = \arcs_{\reachGraph} \cup \{(m_2,l,m_f)\}$;% \tcp{Replace arc from the source of the arc, its label and the target marking of the $\tau$ arc}
     }
     $\arcs_{\reachGraph} = \arcs_{\reachGraph} \setminus \{(m_1,\tau,m_f)\}$; \tcp{Remove the $\tau$ arc from the reachability graph}
 }
 \caption{Remove Tau Transitions}\label{alg:remTau}
}
\end{algorithm}
\setlength{\textfloatsep}{\baselineskip}

%As we mentioned before, $\tau$ transitions are not recorded in an event log, hence they can be removed from the reachability graph $\reachGraph$.
Petri nets can contains $\tau$-transitions representing invisible steps that are not recorded in an event log and they are captured in the reachability graph of a Petri net. Our technique aims at matching events from the event log to activities in the process model, and thus $\tau$ transitions can never be matched. Other techniques like \cite{AdriansyahDA11,BVD-Alignment} handle these $\tau$-transitions as automatically matched events. We argue however that a pre-emptive removal of $\tau$ transitions from the reachability graph can speed up the presented technique since less steps need to be considered.
%which decreases the searchspace.
In principle, we assume that a Petri net has a minimal number of $\tau$-transitions, for instance, by applying structural reduction rules that preserve all visible behavior~\cite{murata}. However not all $\tau$-transitions can be removed by structural reduction of the Petri net. We therefore remove the remaining $\tau$-transitions through behavior preserving reduction rules on the reachability graph by the breadth-first search algorithm given in Alg.~\ref{alg:remTau}.
%\footnote{While the $\tau$-transitions could also be removed from the Petri net, this would lead to model transformations (e.g. transition duplications) which would in turn lead to a state explosion of the reachability graph.}.
Intuitively, for every marking $m$ reached by a $\tau$-transition $a_1 = (m_1,\tau,m) \in \arcs_{\reachGraph}$ and any outgoing transition $a_2 = (m,l,m_2) \in A_R$, the algorithm replaces $a_1$ with $a_{12} = (m_1,l,m_2)$ (lines 6-8 and lines 19-21).
%In doing so, it changes the source of all duplicate arcs to the source of $a$.
This replacement is repeated until all arcs representing $\tau$-transitions are removed. In case all incoming arcs of a state get replaced we also remove $m$ and its outgoing arcs (Lines 12-16). Function $\emph{replaceTau}$ also handles the case of another outgoing $\tau$-labeled transition $a_2 = (m,\tau,m_2)$ by a depth-first search along $\tau$-transitions in $A_R$ (lines 22-24).
%By construction, the algorithm refrains from removing $\tau$ transitions targeting final markings to ensure proper completion.
The algorithm then removes each remaining $\tau$ transition $a = ( m_1, \tau, m_f )$ targeting the final marking while introducing new replacement arcs $a' = ( m_2, l, m_f )$ for each incoming arc of $m_1$, such that $(m_2,l,m_1) \in \arcs_{\reachGraph}$ (Line 17 and function \emph{replaceTauBackwards}).
The reachability graph returned by Alg.~\ref{alg:remTau} is now free of $\tau$ transitions.
Figure~\ref{fig:modelFSM} shows the $\tau$-less reachability graph of the loan application process.
%Starting from reachability graph all arcs with invisible task labels are replaced with the outgoing arcs of their target
Observe that the node $[p1,p2,p3,p4]$ is removed and its outgoing arcs are connected to the node $[start]$, and, similarly, node $[p5,p6,p7,p8]$ is removed and its incoming arcs now target the node $[p9]$ instead. %As can be easily checked, the tau-less reachability graph preserves all behavior allowed by the Petri Net while removing invisible tasks.
In addition, the arc $([p11],\tau,[\text{end}])$ is replaced with the newly introduced arc $([p10],G,[\text{end} ])$.

